The Bees Algorithm for the Vehicle Routing Problem

In this thesis we present a new algorithm for the Vehicle Routing Problem called the Enhanced Bees Algorithm. It is adapted from a fairly recent algorithm, the Bees Algorithm, which was developed for continuous optimisation problems. We show that the results obtained by the Enhanced Bees Algorithm are competitive with the best meta-heuristics available for the Vehicle Routing Problem (within 0.5% of the optimal solution for common benchmark problems). We show that the algorithm has good runtime performance, producing results within 2% of the optimal solution within 60 seconds, making it suitable for use within real world dispatch scenarios.

==> implementation.tex <==
%!TEX root = main.tex

% =====================
% CHAPTER
% ---------------------
% =====================
\chapter{Appendix A - Implementation}
This chapter details how the optimization system is implemented. The system's architecture, technologies employed in the system and optimisations done to the system are detailed here.

% =====================
% Implementation goals
% =====================
\section{Parallelization}

Actor Model

\section{Source Code}

Get it here ...


